Pretraining on Interactions for Learning Grounded Affordance Representations

Lexical semantics and cognitive science point to affordances (i.e. the actions that objects support) as critical for understanding and representing nouns and verbs. However, study of these semantic features has not yet been integrated with the "foundation" models that currently dominate language representation research. We hypothesize that predictive modeling of object state over time will result in representations that encode object affordance information "for free". We train a neural network to predict objects' trajectories in a simulated interaction and show that our network's latent representations differentiate between both observed and unobserved affordances. We find that models trained using 3D simulations from our SPATIAL dataset outperform conventional 2D computer vision models trained on a similar task, and, on initial inspection, that differences between concepts correspond to expected features (e.g., roll entails rotation). Our results suggest a way in which modern deep learning approaches to grounded language learning can be integrated with traditional formal semantic notions of lexical representations.

==> sections/discussion.tex <==
\section{Discussion and Future Work}
In this study, we find that training on 3D spatial data consistently outperforms training on 2D visual data, and that pretraining often (but not always) improves over a randomly-initialized model. The counterfactual analysis in Section \ref{sec:error_analysis} further suggests that our proposed approach of 3D pretraining might learn to distinguish actions for the "right" reasons. These results are exciting, as they suggest a path forward for work that asks if and how neural approaches can automatically learn lexical semantic concepts. The models proposed are only a starting point--their performance still falls short of what we'd ultimately hope to achieve as part of a general langauge-learning system. Even so, our work provides novel evidence of the advantages of using 3D spatial data over 2D pixel data in learning effective affordance representations. These ideas, along with the release of the \ours\ dataset, provide a starting point for further research where pretraining objectives can be augmented to include richer notions of embodiment (e.g., planning, agent-agent interaction) and perhaps consequently encode richer lexical semantic structure (e.g., presuppositions, transitivity).

==> sections/results.tex <==
\section{Results}
For now all of this is in the experiments section

\subsection{Error Analysis}
TODO: We expect to see the model has an easier time predicting affordances of the unseen objects that are 'easier'...
